Uncovering the Interaction Equation: Quantifying the Effect of User Interactions on Social Media Homepage Recommendations

Social media platforms depend on algorithms to select, curate, and deliver content personalized for their users. These algorithms leverage users' past interactions and extensive content libraries to retrieve and rank content that personalizes experiences and boosts engagement. Among various modalities through which this algorithmically curated content may be delivered, the homepage feed is the most prominent. This paper presents a comprehensive study of how prior user interactions influence the content presented on users' homepage feeds across three major platforms: YouTube, Reddit, and X (formerly Twitter). We use a series of carefully designed experiments to gather data capable of uncovering the influence of specific user interactions on homepage content. This study provides insights into the behaviors of the content curation algorithms used by each platform, how they respond to user interactions, and also uncovers evidence of deprioritization of specific topics.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

all 	: $(TRG)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 

include $(SRC:.tex=.d)

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@

#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
#$(PDF) : %.pdf : %.tex
#	@$(run-pdflatex)


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))


==> sections/results.tex <==
\section{Results}

% \begin{table}[h!]
% \centering
% \begin{tabular}{lccc}
% \toprule
% Platform & NFL & Elections & Fitness \\
% \midrule
% Reddit & 3.63 & 0.72 & 2.07 \\
% YouTube & 2.07 & 4.33 & 1.39 \\
% Twitter & 0.40 & -0.06 & 0.29 \\
% \bottomrule
% \end{tabular}
% \caption{\textbf{Topic Influence}.Average influence of each topic across actions and positions on homepage compositions. *Indicates a significantly higher change in homepage composition compared to other topics. \note{added to table}}
% \end{table}
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}

% \begin{table}[h!]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lrrrrrrrrrrrr@{}}
% \toprule
% \textbf{F values} & \textbf{control} & \textbf{follow} & \textbf{join} & \textbf{like} & \textbf{open} & \textbf{search} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{P1} & \textbf{P2} & \textbf{P3} \\ \midrule
% \textbf{YouTube}  & 0.18             & 3.00            & -             & 36.52         & 1.87          & 0.50            & 6.19               & 0.80             & 3.70         & 3.79        & 2.70        & 1.79        \\
% \textbf{Reddit}   & 0.24             & -               & 301.06        & 0.85          & 0.72          & 0.23            & 0.78               & 1.95             & 6.77         & 4.33        & 2.05        & 1.17        \\
% \textbf{Twitter}  & 0.90             & 1.54            & 0.83          & 2.16          & 0.76          & 0.64            & 0.83               & 1.19             & 1.23         & 1.43        & 0.93        & 0.90        \\ \bottomrule
% \end{tabular}%
% }
% \caption{\textbf{Fvalues} for the system of equations.}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
%  & \textbf{search} & \textbf{like} & \textbf{follow} & \textbf{join} & \textbf{open} & \textbf{control} \\ \midrule
% \textbf{YouTube} & 0.04 & 28.61* & 12.62* & -& 23.25* & 0.0 \\
% \textbf{Twitter} & -3.2 & 7.44* & 5.68* & 0.73 & -0.72 & 0.0 \\
% \textbf{Reddit} & 0.12 & 3.57 & -& 26.83* & 3.74* & 0.0 \\ \bottomrule
% \end{tabular}
% \caption{\textbf{Average treatment effect on ranked homefeed.} Comparing the influence of each action with the control action for the first dosage. * Indicates significantly greater influence compared to the control action. \note{added to table}}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
%  & \textbf{search} & \textbf{like} & \textbf{follow} & \textbf{join} & \textbf{open} & \textbf{control} \\ \midrule
% \textbf{YouTube} & 0.43 & 21.25* & 4.34* & -& 17.49* & 0.0 \\
% \textbf{Twitter} & -0.83 & 2.72& 2.6* & 0.36 & 0.6 & 0.0 \\
% \textbf{Reddit} & 0.36 & 3.26*& -& 21.72* & 4.22* & 0.0 \\ \bottomrule
% \end{tabular}
% \caption{\textbf{Average treatment effect on feeds.} Comparing the influence of each action with the control action for the first dosage. * Indicates significantly greater influence compared to the control action. \note{added to table}}
% \end{table}



% \begin{table}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{rrrrrrrrrrrrrrrr} 
% \multicolumn{1}{l}{} & \multicolumn{3}{c}{\textbf{Search}}                  & \multicolumn{3}{c}{\textbf{Like}}                    & \multicolumn{3}{c}{\textbf{Follow}}                  & \multicolumn{3}{c}{\textbf{Join}}                    & \multicolumn{3}{c}{\textbf{Open}}                    \\ 
% \textbf{}            & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} \\ 
% \textbf{YouTube}     & 0.71         & 2.65               & 0.9              & 22.61*       & 34.39*             & 13.78*           & 5.13*        & 6.4*               & 4.51             & -            & -                  & -                & 20.05*       & 20.98*             & 14.95*           \\ 
% \textbf{Twitter}     & 0.02         & -1.91              & 0.42             & 3.91         & -2.32              & 6.03*            & 6.87*        & 2.31               & 3.54             & 0.41         & -0.12              & 1.75             & 0.7          & 0.15               & 1.74             \\ 
% \textbf{Reddit}      & 1.98         & 0.86               & 0.27             & 10.59*       & -0.33              & -0.04            & -            & -                  & -                & 28.37*       & 28.35*             & 12.29*           & 10.75*       & 3.63*              & 2.21            
%  \\ \end{tabular}}
% \caption{Average treatment effect of action and topic pairs on \textbf{topic}. Comparing the influence of each treatment with corresponding control treatment for its first dosage. * Indicates significantly greater influence compared to the control action. \note{added to table}} 
% \end{table}

% \begin{table}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{rrrrrrrrrrrrr}
% \multicolumn{1}{l}{} & \multicolumn{3}{c}{\textbf{Like}}                    & \multicolumn{3}{c}{\textbf{Follow}}                  & \multicolumn{3}{c}{\textbf{Join}}                    & \multicolumn{3}{c}{\textbf{Open}}                    \\
% \textbf{}            & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} \\
% \textbf{YouTube}     & 30.24*       & 41.65*             & 19.43*           & 10.15*       & 18.09*             & 12.28*           & nan          & nan                & nan              & 27.21*       & 26.68*             & 17.86*           \\
% \textbf{Twitter}& 16.38        & -7.33              & 14.03*           & 17.79*       & -0.14              & 1.81             & 5.33         & -2.12              & 3.7              & 2.23         & 0.89               & 0.82             \\
% \textbf{Reddit}      & 13.08*       & -3.72              & -0.02            & nan          & nan                & nan              & 34.56*       & 29.24*             & 18.61*           & 10.47*       & 1.62*              & 0.0             
% \end{tabular}
% }
% \caption{Average treatment effect of action and topic pairs on \textbf{topic} (\textbf{ranked}). Comparing the influence of each treatment with corresponding control treatment for its first dosage. * Indicates significantly greater influence compared to the control action. \note{added to table.}} 
% \end{table}

% \begin{table}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{rrrrrrrrrrrrr}
% \multicolumn{1}{l}{} & \multicolumn{3}{c}{\textbf{Search}}                  & \multicolumn{3}{c}{\textbf{Follow}}                  & \multicolumn{3}{c}{\textbf{Join}}                    & \multicolumn{3}{c}{\textbf{Open}}                    \\
% \textbf{}            & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} \\
% \textbf{YouTube}     & 2.34         & 7.41               & 3.4              & 1.82         & 6.72               & 4.13             & nan          & nan                & nan              & 0.27         & -5.24              & -0.94            \\
% \textbf{Twitter}& 5.34         & 0.22               & 0.23             & 6.41         & 0.0                & 0.7              & 0.0          & 0.0                & 0.0              & 0.0          & 0.0                & 0.78             \\
% \textbf{Reddit}      & 0.0          & 0.0                & 0.0              & nan          & nan                & nan              & 26.83        & 37.3               & 12.5             & 0.0          & 0.0                & 0.0             
% \end{tabular}
% }
% \caption{Average treatment effect of action and topic pairs on \textbf{source}. Comparing the influence of each treatment with corresponding control treatment for its first dosage on source. * Indicates significantly greater influence compared to the control action.} 
% \label{tab:my_table}
% \end{table}
% \begin{table}[h!]
% \centering
% \begin{tabular}{@{}lrrrrr@{}}
% \toprule
%  & \textbf{follow} & \textbf{join} & \textbf{like} & \textbf{open} & \textbf{control} \\ \midrule
% \textbf{YouTube} & 3.59 & -& 2.93 & 0.49& 0.01\\
% \textbf{Twitter} & 0.78 & 0.0 & 0.99 & 0.18 & 0.0\\
% \textbf{Reddit} & -& 14.56 & 0.1 & 0.0& 0.0 \\ \bottomrule
% \end{tabular}
% \caption{\textbf{Average treatment effect on sources 
% within feeds.} Percentage of interacted source before - Percentage of interacted source after.}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
%  & \textbf{search} & \textbf{like} & \textbf{follow} & \textbf{join} & \textbf{open} & \textbf{control} \\ \midrule
% \textbf{YouTube} & 0.17 & 1.42* & 0.28 & -& 1.06* & 0.0 \\
% \textbf{Reddit} & -0.0 & 0.14 & -& 1.59* & 0.19* & 0.0 \\
% \textbf{Twitter} & 0.0 & 0.39* & 0.22 & 0.13 & 0.03 & 0.0 \\ \bottomrule
% \end{tabular}
% \caption{\textbf{Average treatment effect on homepage centroid.} Difference of centroid shift for each action from the centroid shift of the control action (for first dose actions only). Centroid shift is calculated using the Euclidean distances between pre- and post-treatment homepages centroid. \note{added to table}}
% \end{table}

% \begin{table}
% \centering

% \begin{tabular}{r r r}
%  & Avg. \% of in network posts&Std. Dev\\
% Reddit& 45.85\%& 16.46\\
% Twitter & 1.30\%& 1.50\\
% YouTube & 13.38\%& 6.49\\

% \end{tabular}
% \caption{\textbf{Percentage of posts from subscribed sources}}
% \end{table}


% \section{Dosage effect}
% \note{Code: algoanalyst/src/1. Is there a dosage effect?.ipynb}
% \note{\textit{config}: across all actions, all topics, all positions. Change calculated using topic\_1 Jaccard.}
% \note{Updated: These are now \textbf{influence} on homepage \textbf{topic composition}: how does liking A change the percentage of A in homepage.} 

% \begin{table}[]
% \begin{tabular}{@{}lrr@{}}
% \toprule
%                  & \multicolumn{1}{l}{\textbf{Dosage Effect}} & \multicolumn{1}{l}{\textbf{Position Effect}} \\ \midrule
% \textbf{YouTube} & -2.01*                                     & -0.35                                        \\
% \textbf{Reddit}  & -1.44*                                     & -0.85*                \\
% \textbf{Twitter} & -0.40*                                     &  -0.29                 \\ \bottomrule
% \end{tabular}
% \caption{\textbf{Regression ordinals.} Values represent the regression value of the dosage and position effect as the dosage/position increases. * indicates significance.}
% \end{table}

% \begin{table}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{rrrrrrrrrrrrrrrrrrrrrr}
% \multicolumn{1}{l}{} & \multicolumn{3}{l}{\textbf{Search}}     & \multicolumn{3}{l}{\textbf{Like}}       & \multicolumn{3}{l}{\textbf{Follow}}     & \multicolumn{3}{l}{\textbf{Join}}       & \multicolumn{3}{l}{\textbf{Open}}       & \multicolumn{3}{l}{\textbf{Control}}    & \multicolumn{3}{l}{\textbf{All Actions}} \\
% \textbf{}            & \textbf{Y1} & \textbf{Y2} & \textbf{Y3} & \textbf{Y1} & \textbf{Y2} & \textbf{Y3} & \textbf{Y1} & \textbf{Y2} & \textbf{Y3} & \textbf{Y1} & \textbf{Y2} & \textbf{Y3} & \textbf{Y1} & \textbf{Y2} & \textbf{Y3} & \textbf{Y1} & \textbf{Y2} & \textbf{Y3} & \textbf{Y1}  & \textbf{Y2} & \textbf{Y3} \\
% YouTube              & 0.23        & 0.61        & -0.02       & 4.94        & 7.80        & 5.31        & 3.24        & 3.74        & 3.29        & -           & -           & -           & 2.37        & 3.35        & 2.84        & 0.01        & 0.43        & 0.29        & 2.26         & 3.39        & 2.4         \\
% Twitter              & -0.16       & -0.19       & -0.63       & 3.19        & 1.38        & -0.03       & 1.26        & 0.80        & 0.68        & 0.39        & -0.24       & 0.07        & 0.10        & -0.45       & -0.62       & 0.14        & -0.02       & -0.02       & 0.7          & 0.23        & -0.14       \\
% Reddit               & 0.03        & 0.31        & -0.06       & 2.65        & 0.67        & 2.01        & -           & -           & -           & 11.67       & 6.96        & 4.71        & 3.60        & 0.13        & 1.75        & 0.08        & 0.35        & -0.02       & 3.74         & 1.9         & 1.82       
% \end{tabular}
% }
% \caption{Y1, Y2, Y3 values} Here Y1 is NFL, Fitness Elections. Y2: Fitness, Elections, NFL. Y3: Elections Fitness, NFL. Pvalues in the table below

% \end{table}

% \begin{table}[]
% \begin{tabular}{rrrrrrrl}
% \textbf{} & \textbf{search} & \textbf{like} & \textbf{follow} & \textbf{join} & \textbf{open} & \textbf{control}& \textbf{All actions} \\
% YouTube   & 0.655           & 0.511         & 0.845           & nan           & 0.933         & 0.901     & 0.33                 \\
% Twitter   & 0.699           & 0.348         & 0.638           & 0.548         & 0.181         & 0.970     & 0.20                 \\
% Reddit    & 0.561           & 0.269         & nan             & 0.104         & \textbf{0.005}         & 0.513     & \textbf{0.04}\end{tabular}
% \caption{\textbf{Pvalues for Y1 = Y2 = Y3}}
% \end{table}

% \begin{table}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{rrrrrrrrrrrrrrrr}
% \multicolumn{1}{l}{} & \multicolumn{3}{l}{\textbf{Search}}                  & \multicolumn{3}{l}{\textbf{Like}}                    & \multicolumn{3}{l}{\textbf{Follow}}                  & \multicolumn{3}{l}{\textbf{Join}}                    & \multicolumn{3}{l}{\textbf{Open}}                    \\
% \textbf{}            & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} & \textbf{NFL} & \textbf{Elections} & \textbf{Fitness} \\
% \textbf{YouTube}     & 0.29         & -0.0               & 0.24             & 1.50*        & 2.3*               & 0.69*            & 0.23         & 0.16               & 0.42             & nan          & nan                & nan              & 1.6*         & 1.11*              & 0.47*            \\
% \textbf{Reddit}      & -0.0         & 0.03               & -0.0             & 0.26         & 0.18*              & 0.0              & nan          & nan                & nan              & 1.64*        & 2.33*              & 1.06*            & 0.33*        & 0.09               & 0.13             \\
% \textbf{Twitter}     & 0.10         & 0.06               & -0.1             & 0.45*        & 0.44               & 0.27             & 0.74*        & -0.3*              & -0.0             & 0.23         & 0.18               & 0.00             & -0.0         & -0.0               & 0.13            
% \end{tabular}
% }
% \caption{ATE on centroid difference. Measured by calculating difference with correpronding control action \note{added to table}}
% \end{table}

\subsubsection{YouTube} 
\begin{itemize}
    \item \textbf{Yes}, There is a statistically significant decreasing trend in the observations across treatments. 
    \item Linear regression: Coefficient for Treatment\_Ordinal = -0.2687, p-value = 0.0023 
    \item The distributions are significantly different (ANOVA p-value: 0.004).
    \item action specific: 
    \begin{itemize}
        \item Control (no action): no trend.
        \item Search: no trend
        \item Open: Yes, decreasing sig.
        \item Like: yes, decreasing sig.
        \item Follow: yes, decreasing (0.048p)
    \end{itemize}
    \item Topic specific:
    \begin{itemize}
        \item Trend is very sig. decreasing for NFL but not sig  for fitness or elections. (maybe they are too broad?)
        \item Dosage effect true for all positions.
    \end{itemize}
\end{itemize}

\subsubsection{Reddit}
\begin{itemize}
    \item Yes. decreasing trend, signficant.
    \item Like is not sig. decreasing. 
    \item Join is significantly decreasing.
\end{itemize}


\subsubsection{Twitter}
\begin{itemize}
    \item \textbf{Yes!}
    \item There is a statistically significant decreasing trend in the observations across treatments.
    \item  The distributions are significantly different (ANOVA p-value: 0.001).
    \item  Linear regression: Coefficient for Treatment\_Ordinal = -0.4511, p-value = 0.0002
    \item Actions:
    \begin{itemize}
        \item Like: sig decreasing trend
        \item Follow: no sig decreasing trend
    \end{itemize}
\item Topics:
\begin{itemize}
    \item Fitness and NFL are sig decreasing. Elections is not.
\end{itemize}
\end{itemize}

\subsubsection{thoughts}
\begin{enumerate}
    \item Now that we have identified a trend (or even a decay curve for dosage) can we reomove it? if so, how?
    \item All platforms on control actions (no action) show no decreasing trend. Is there any reason to incorporate this control trend to account for time? observation influence?
    \item Should we incorporate noise actions into this?
\end{enumerate}


\subsubsection{some good things}
\begin{itemize}
    \item all control actions (no actions) show no trend. Validates our method somewhat.
    \item No search has trends
    \item For twitter and reddit follow does not have a sig decreasing trend, but like does. That makes sense. follow is a network source and like is an inference source. Liking 10th nfl post might not have an effect but following 10th nfl user still would result in that user showing up. Maybe there is a threshold to the number of users tho. At max we follow 9 users (across topics).
\end{itemize}

\section{Position decay curve}

Only reddit has a decreasing trend (specifically for liking). Other platforms do not have a decay curve.


\subsection{Are all topics same?}
Is the influence of action the same across different topics?
Method: get all \textit{influence of action} after each topic separately. are the distributions significantly different?
For our analysis this would imply that we can use all signals to measure the influence of actions.


\subsection{Is there a recency bias}
No. The composition of the homepage is not dominated by the most recent interaction. Investigating ranking bias in ranking yields similar results.
